Towards Digital Nature: Bridging the Gap between Turing Machine Objects and Linguistic Objects in LLMMs for Universal Interaction of Object-Oriented Descriptions

In this paper, we propose a novel approach to establish a connection between linguistic objects and classes in Large Language Model Machines (LLMMs) such as GPT3.5 and GPT4, and their counterparts in high level programming languages like Python. Our goal is to promote the development of Digital Nature: a worldview where digital and physical realities are seamlessly intertwined and can be easily manipulated by computational means. To achieve this, we exploit the inherent abstraction capabilities of LLMMs to build a bridge between human perception of the real world and the computational processes that mimic it. This approach enables ambiguous class definitions and interactions between objects to be realized in programming and ubiquitous computing scenarios. By doing so, we aim to facilitate seamless interaction between Turing Machine objects and Linguistic Objects, paving the way for universally accessible object oriented descriptions. We demonstrate a method for automatically transforming real world objects and their corresponding simulations into language simulable worlds using LLMMs, thus advancing the digital twin concept. This process can then be extended to high level programming languages, making the implementation of these simulations more accessible and practical. In summary, our research introduces a groundbreaking approach to connect linguistic objects in LLMMs with high level programming languages, allowing for the efficient implementation of real world simulations. This ultimately contributes to the realization of Digital Nature, where digital and physical worlds are interconnected, and objects and simulations can be effortlessly manipulated through computational means.

==> jscodes/cat.tex <==
\begin{lstlisting}[caption=cat.js,label=catjs]
export class Cat {
  constructor() {
    this.mainObj = {
      name: "cat",
      subObjList: [
        {
          type: "skill",
          list: ["jump", "climb", "hunt", "purr", "scratch", "meow"]
        },
        {
          type: "knowledge",
          list: ["anatomy", "behavior", "diet", "predators", "domestication", "communication"]
        },
        {
          type: "state",
          list: ["hungry", "resting", "playing", "grooming", "communicating"]
        },
        {
          type: "stateDetection",
          list: [
            {
              state: "hungry",
              condition: (energy, lastMealTime, activity, cleanliness, socialInteraction, lastSocialInteraction) => energy < 50 || lastMealTime > 4
            },
            {
              state: "resting",
              condition: (energy, lastMealTime, activity, cleanliness, socialInteraction, lastSocialInteraction) => energy >= 50 && activity === "inactive"
            },
            {
              state: "playing",
              condition: (energy, lastMealTime, activity, cleanliness, socialInteraction, lastSocialInteraction) => energy >= 50 && activity === "active"
            },
            {
              state: "grooming",
              condition: (energy, lastMealTime, activity, cleanliness, socialInteraction, lastSocialInteraction) => energy >= 50 && cleanliness < 80
            },
            {
              state: "communicating",
              condition: (energy, lastMealTime, activity, cleanliness, socialInteraction, lastSocialInteraction) => socialInteraction === true && lastSocialInteraction > 2
            }
          ]
        },
        {
          type: "skillExecution",
          list: [
            {
              skill: "jump",
              action: (object) => {
                console.log("The cat jumps.");
                // Move the cat object in the 3D world using Three.js
                object.position.y += 0.05;
                object.position.z -= 0.05;
              }
            },
            {
              skill: "climb",
              action: (object) => {
                console.log("The cat climbs.");
                // Move the cat object in the 3D world using Three.js
                object.position.y += 0.1;
              }
            },
            {
              skill: "hunt",
              action: (object) => {
                console.log("The cat hunts.");
                // Move the cat object in the 3D world and interact with other objects using Three.js
                object.position.x += 0.05;
                object.position.z += 0.05;
              }
            },
            {
              skill: "purr",
              action: (object) => {
                console.log("The cat purrs.");
                // Change the cat object's animation in the 3D world using Three.js
                // Note: Assuming the cat object has an animation mixer and purr animation
                // object.animationMixer.clipAction(object.animations.purr).play();
              }
            },
            {
              skill: "scratch",
              action: (object) => {
                console.log("The cat scratches.");
                // Move the cat object in the 3D world and interact with other objects using Three.js
                object.position.x -= 0.05;
                object.position.z += 0.05;
              }
            },
            {
              skill: "meow",
              action: (object) => {
                console.log("The cat meows.");
                // Emit sound from the cat object in the 3D world using Three.js
                // Note: Assuming a meow sound is loaded as an audio buffer and the audioListener is set up
                // const audio = new THREE.Audio(object.audioListener);
                // audio.setBuffer(object.meowSound);
                // audio.play();
              }
            }
          ]
        }
      ]
    };

    this.managerObj = {
      mainObj: this.mainObj,
      currentState: "resting",
      energy: 100,
      lastMealTime: 0,
      activity: "inactive",
      cleanliness: 100,
      socialInteraction: false,
      lastSocialInteraction: 0,
      position: { x: 0, y: 0, z: 0 },
      // boundingBox: { width: 20, height: 10, depth: 20 }
      boundingBox: { width: 10, height: 5, depth: 10 }
    };
  }

  validateState(state) {
    let validStates = this.mainObj.subObjList.find(obj => obj.type === "state").list;
    return validStates.includes(state);
  }

  updateManagerObjState() {
    let stateDetectionList = this.managerObj.mainObj.subObjList.find(
      obj => obj.type === "stateDetection"
    ).list;

    for (let detection of stateDetectionList) {
      if (
        detection.condition(
          this.managerObj.energy,
          this.managerObj.lastMealTime,
          this.managerObj.activity,
          this.managerObj.cleanliness,
          this.managerObj.socialInteraction,
          this.managerObj.lastSocialInteraction
        )
      ) {
        this.managerObj.currentState = detection.state;
        break;
      }
    }
  }

  generateStepObjList() {
    let stepObjList = [];
    let skillExecutionList = this.managerObj.mainObj.subObjList.find(
      obj => obj.type === "skillExecution"
    ).list;

    if (this.managerObj.currentState === "hungry" || this.managerObj.currentState === "grooming") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "hunt"));
    } else if (this.managerObj.currentState === "playing") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "jump"));
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "climb"));
    } else if (this.managerObj.currentState === "resting") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "purr"));
    } else if (this.managerObj.currentState === "communicating") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "meow"));
    }

    return stepObjList;
  }
}


export function updateCatPerFrame(catAloInstance, catObject) {
  catAloInstance.updateManagerObjState();

  const stepObjList = catAloInstance.generateStepObjList();
  for (const stepObj of stepObjList) {
    stepObj.action(catObject);
  }

  // Update cat's energy, lastMealTime, cleanliness, and lastSocialInteraction
  catAloInstance.managerObj.energy -= 0.01;
  catAloInstance.managerObj.lastMealTime += 0.01;
  catAloInstance.managerObj.cleanliness -= 0.005;
  catAloInstance.managerObj.lastSocialInteraction += 0.01;

  // Keep the cat within the boundaries of the bounded 3D physical world
  const boundaries = catAloInstance.managerObj.boundingBox;
  catObject.position.x = Math.max(
    Math.min(catObject.position.x, boundaries.width / 2),
    -boundaries.width / 2
  );
  catObject.position.y = Math.max(
    Math.min(catObject.position.y, boundaries.height / 2),
    -boundaries.height / 2
  );
  catObject.position.z = Math.max(
    Math.min(catObject.position.z, boundaries.depth / 2),
    -boundaries.depth / 2
  );
}
\end{lstlisting}

==> jscodes/roomba.tex <==
\begin{lstlisting}[caption=roomba.js,label=roombajs]
export class Roomba {
  constructor(position, boundingBox, dockPosition, scene) {
    this.mainObj = {
      name: "roomba",
      subObjList: []
    };

    this.mainObj.subObjList = [
      {
        type: "skill",
        list: ["moveForward", "rotate", "detectObstacle", "changeDirection", "clean", "returnToDock"]
      },
      {
        type: "knowledge",
        list: ["navigation", "batteryManagement", "cleaningMechanism", "obstacleDetection", "dockingStation"]
      }
    ];

    this.mainObj.subObjList.push({
      type: "state",
      list: ["idle", "cleaning", "obstacleDetected", "returningToDock", "charging"]
    });

    this.mainObj.subObjList.push({
      type: "stateDetection",
      list: [
        {
          state: "idle",
          condition: (battery, cleaningStatus) => battery >= 20 && cleaningStatus === "notInProgress"
        },
        {
          state: "cleaning",
          condition: (battery, cleaningStatus) => battery >= 20 && cleaningStatus === "inProgress"
        },
        {
          state: "obstacleDetected",
          condition: (obstacle) => obstacle !== null
        },
        {
          state: "returningToDock",
          condition: (battery, cleaningStatus) => battery < 20 && cleaningStatus === "notInProgress"
        },
        {
          state: "charging",
          condition: (battery, docked) => battery < 100 && docked === true
        }
      ]
    });

    this.mainObj.subObjList.push({
      type: "skillExecution",
      list: [
        {
          skill: "moveForward",
          action: (object, distance) => {
            console.log("The Roomba moves forward.");
            const forwardDirection = new THREE.Vector3(Math.sin(object.rotation.y), 0, -Math.cos(object.rotation.y));
            object.position.add(forwardDirection.multiplyScalar(distance || 0.1));
          }
        },
        {
          skill: "rotate",
          action: (object, angle) => {
            // console.log(`The Roomba rotates by ${angle} degrees.`);
            object.rotation.y += angle * (Math.PI / 180);
          }
        },
        {
          skill: "detectObstacle",
          action: (object, obstacles) => {
            console.log("The Roomba detects an obstacle.");
            const detectionDistance = 1;
            let obstacleDetected = false;
        
            for (let obstacle of obstacles) {
              const distance = object.position.distanceTo(obstacle.position);
              if (distance <= detectionDistance) {
                obstacleDetected = true;
                break;
              }
            }
        
            return obstacleDetected;
          }
        },

        {
          skill: "changeDirection",
          action: (object) => {
            console.log("The Roomba changes direction.");
            const randomAngle = Math.random() * 360;
            object.rotation.y += randomAngle * (Math.PI / 180);
          }
        },
        {
          skill: "clean",
          action: (object) => {
            console.log("The Roomba cleans the area.");
            // object.cleaningMechanism.rotation.z += 0.1;
          }
        },
        {
          skill: "returnToDock",
          action: (object, dockPosition) => {
            console.log("The Roomba returns to its docking station.");
            const direction = dockPosition.clone().sub(object.position).normalize() / 100.;
            object.position.add(direction);
          }
        }
      ]
    });

    this.managerObj = {
      mainObj: this.mainObj,
      currentState: "idle",
      battery: 100,
      cleaningStatus: "notInProgress",
      docked: false,
      obstacle: null,
      position: position || { x: 0, y: 0, z: 0 },
      boundingBox: boundingBox || { width: 20, height: 10, depth: 20 },
      dockPosition: dockPosition || { x: 10, y: 0, z: 10 }
    };
  }

  validateState(state) {
    let validStates = this.managerObj.mainObj.subObjList.find(obj => obj.type === "state").list;
    return validStates.includes(state);
  }

  updateManagerObjState() {
    let stateDetectionList = this.managerObj.mainObj.subObjList.find(
      obj => obj.type === "stateDetection"
    ).list;

    for (let detection of stateDetectionList) {
      let conditionResult;
      switch (detection.state) {
        case "idle":
        case "cleaning":
        case "returningToDock":
          conditionResult = detection.condition(
            this.managerObj.battery,
            this.managerObj.cleaningStatus
          );
          break;
        case "obstacleDetected":
          conditionResult = detection.condition(this.managerObj.obstacle);
          break;
        case "charging":
          conditionResult = detection.condition(this.managerObj.battery, this.managerObj.docked);
          break;
      }

      if (conditionResult) {
        this.managerObj.currentState = detection.state;
        break;
      }
    }
  }

  generateStepObjList() {
    let stepObjList = [];
    let skillExecutionList = this.managerObj.mainObj.subObjList.find(
      obj => obj.type === "skillExecution"
    ).list;

    if (this.managerObj.currentState === "idle" || this.managerObj.currentState === "cleaning") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "moveForward"));
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "rotate"));
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "detectObstacle"));
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "clean"));
    } else if (this.managerObj.currentState === "obstacleDetected") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "changeDirection"));
    } else if (this.managerObj.currentState === "returningToDock") {
      stepObjList.push(skillExecutionList.find(skill => skill.skill === "returnToDock"));
    }

    return stepObjList;
  }
}

export function updateRoombaPerFrame(roomba, roombaObject, scene, obstacles) {
  // Update the managerObj state
  roomba.updateManagerObjState();

  // Generate the stepObjList based on the current state
  const stepObjList = roomba.generateStepObjList();

  // Execute the actions in the stepObjList
  for (const stepObj of stepObjList) {
    switch (stepObj.skill) {
      case "moveForward":
        stepObj.action(roombaObject);
        break;
      case "rotate":
        // const angle = Math.random() * 360;
        // stepObj.action(roombaObject, angle);
        stepObj.action(roombaObject, 1.);
        break;
      case "detectObstacle":
        roomba.managerObj.obstacle = stepObj.action(roombaObject, obstacles) ? "detected" : null;
        break;
      case "changeDirection":
        stepObj.action(roombaObject);
        break;
      case "clean":
        stepObj.action(roombaObject);
        break;
      case "returnToDock":
        stepObj.action(roombaObject, roomba.managerObj.dockPosition);
        break;
    }
  }

  // Check for collisions with scene objects
  const box = new THREE.Box3().setFromObject(roombaObject);
  for (const object of scene.children) {
    if (object !== roombaObject && box.intersectsBox(new THREE.Box3().setFromObject(object))) {
      roomba.managerObj.obstacle = "detected";
      break;
    }
  }
}
\end{lstlisting}

==> jscodes/world.tex <==
\begin{lstlisting}[caption=world.js,label=worldjs]
export class Bounded3DPhysicalWorld {
  constructor() {
    this.mainObj = {
      name: "bounded3DPhysicalWorld",
      subObjList: [
        {
          type: "skill",
          list: [
            "createObject",
            "moveObject",
            "rotateObject",
            "scaleObject",
            "removeObject",
            "changeMaterial",
            "addLight",
          ],
        },
        {
          type: "knowledge",
          list: [
            "coordinateSystem",
            "physics",
            "materials",
            "lighting",
            "collisionDetection",
            "textures",
            "shadows",
            "boundaries",
          ],
        },
        {
          type: "state",
          list: [
            "idle",
            "objectCreation",
            "objectManipulation",
            "objectRemoval",
            "materialChange",
            "lightingAdjustment",
          ],
        },
        {
          type: "stateDetection",
          list: [
            {
              state: "idle",
              condition: (selectedObject) => selectedObject === null,
            },
            {
              state: "objectCreation",
              condition: (action) => action === "createObject",
            },
            {
              state: "objectManipulation",
              condition: (selectedObject, action) =>
                selectedObject !== null &&
                ["moveObject", "rotateObject", "scaleObject"].includes(action),
            },
            {
              state: "objectRemoval",
              condition: (selectedObject, action) =>
                selectedObject !== null && action === "removeObject",
            },
            {
              state: "materialChange",
              condition: (selectedObject, action) =>
                selectedObject !== null && action === "changeMaterial",
            },
            {
              state: "lightingAdjustment",
              condition: (selectedObject, action) =>
                selectedObject !== null && action === "addLight",
            },
          ],
        },
        {
          type: "skillExecution",
          list: [
            {
              skill: "createObject",
              action: (objectType) =>
                console.log(
                  `A new ${objectType} is created in the bounded 3D physical world.`
                ),
            },
            {
              skill: "moveObject",
              action: (object, newPosition) =>
                console.log(
                  `The ${object} is moved to the new position: ${newPosition}.`
                ),
            },
            {
              skill: "rotateObject",
              action: (object, newRotation) =>
                console.log(
                  `The ${object} is rotated to the new rotation: ${newRotation}.`
                ),
            },
            {
              skill: "scaleObject",
              action: (object, newScale) =>
                console.log(
                  `The ${object} is scaled to the new scale: ${newScale}.`
                ),
            },
            {
              skill: "removeObject",
              action: (object) =>
                console.log(
                  `The ${object} is removed from the bounded 3D physical world.`
                ),
            },
            {
              skill: "changeMaterial",
              action: (object, newMaterial) =>
                console.log(
                  `The ${object} has its material changed to: ${newMaterial}.`
                ),
            },
            {
              skill: "addLight",
              action: (lightType, position) =>
                console.log(
                  `A new ${lightType} is added to the bounded 3D physical world at position: ${position}.`
                ),
            },
          ],
        },
      ],
    };

    this.managerObj = {
      mainObj: this.mainObj,
      currentState: "idle",
      selectedObject: null,
      action: null,
      boundaries: { x: [-100, 100], y: [-100, 100], z: [-100, 100] },
    };
  }

  validateState(state) {
    let validStates = this.mainObj.subObjList.find(
      (obj) => obj.type === "state"
    ).list;
    return validStates.includes(state);
  }

  updateManagerObjState() {
    let stateDetectionList = this.managerObj.mainObj.subObjList.find(
      (obj) => obj.type === "stateDetection"
    ).list;

    for (let detection of stateDetectionList) {
      if (
        detection.condition(
          this.managerObj.selectedObject,
          this.managerObj.action
        )
      ) {
        this.managerObj.currentState = detection.state;
        break;
      }
    }
  }

  generateStepObjList() {
    let stepObjList = [];
    let skillExecutionList = this.managerObj.mainObj.subObjList.find(
      (obj) => obj.type === "skillExecution"
    ).list;

    if (this.managerObj.currentState === "objectCreation") {
      stepObjList.push(
        skillExecutionList.find((skill) => skill.skill === "createObject")
      );
    } else if (this.managerObj.currentState === "objectManipulation") {
      stepObjList.push(
        skillExecutionList.find((skill) => skill.skill === this.managerObj.action)
      );
    } else if (this.managerObj.currentState === "objectRemoval") {
      stepObjList.push(
        skillExecutionList.find((skill) => skill.skill === "removeObject")
      );
    } else if (this.managerObj.currentState === "materialChange") {
      stepObjList.push(
        skillExecutionList.find((skill) => skill.skill === "changeMaterial")
      );
    } else if (this.managerObj.currentState === "lightingAdjustment") {
      stepObjList.push(
        skillExecutionList.find((skill) => skill.skill === "addLight")
      );
    }

    return stepObjList;
  }
}

export function updatePhysicalWorldPerFrame(world) {
  // Update manager object state
  world.updateManagerObjState();

  // Generate step object list for the current state
  let stepObjList = world.generateStepObjList();

  // Execute each step in step object list
  for (let stepObj of stepObjList) {
    stepObj.action();
  }
}
\end{lstlisting}
